Addressing Cross-Lingual Word Sense Disambiguation on Low-Density Languages: Application to Persian

We explore the use of unsupervised methods in Cross-Lingual Word Sense Disambiguation (CL-WSD) with the application of English to Persian. Our proposed approach targets the languages with scarce resources (low-density) by exploiting word embedding and semantic similarity of the words in context. We evaluate the approach on a recent evaluation benchmark and compare it with the state-of-the-art unsupervised system (CO-Graph). The results show that our approach outperforms both the standard baseline and the CO-Graph system in both of the task evaluation metrics (Out-Of-Five and Best result).

==> relatedwork.tex <==
%Persian is a member of the Indo-European language family, and uses Arabic letters for writing. Seraji et al.~\cite{seraji2012} provide a comprehensive overview on the main characteristics of the language. %For instance, the diacritic signs are not written---it is expected that the reader can read the text in the absence of the short vowels. This characteristic causes a special kind of word ambiguity in writing, such that some words are pronounced differently while their written forms are the same. %e.g., \<k^sty> ``wrestling'' and ``ship''.

%In recent years, several tools and libraries were introduced, targeting the complexities of Persian language in NLP. For example, Seraji et al.~\cite{seraji2012} provides a set of tools for preprocessing (Pre-Per), sentence segmentation and tokenization (SeTPer), and also POS tagging (TagPer). Dehdari et al.~\cite{dehdari2008link} brings forward a stemmer and morphological analyzer, called PerStem. More recently, Samvelian et al.~\cite{samvelian2014extending} introduces PersPred, focusing on processing of compounding verbs. Finally, Feely et al.~\cite{feely2014cmu} provides a front-end and new tools for language processing. In this work, similar to Jadidinejad et al.~\cite{jadidinejad2010evaluation}, we use PerStem for stemming, together with TagPer as a state-of-the-art POS tagging tool.

%In addition to the NLP tools, knowledge and data resources are an important part of WSD and CL-WSD solutions. 
%The main knowledge resource in Persian is \emph{FarsNet}~\cite{shamsfard2010semi}---the Persian WordNet. %Its structure is comparable to WordNet and goes by the same principles while containing significantly fewer words ($\sim$13K versus $\sim$147K). Also, most of its synsets are mapped to synsets in WordNet using equal or near-equal relations.
%While the knowledge-based systems are limited and only at high cost extendable to more specific domains, exploiting parallel corpora can be another effective method for CL-WSD. 

Based on our knowledge, the existing parallel corpora (English-Persian) are as follows: Tehran English-Persian Parallel (TEP) ~\cite{pilevar2011tep}, Parallel English-Persian News (PEN)~\cite{farajian2011pen}, and the European Language Resource Association (ELRA) corpus. Among the mentioned resources, TEP is the only freely available one, but it is only a small set of informal conversations in movie subtitles, and therefore it is not sufficient for a general representation of the language.

In the absence of reliable and comprehensive resources, our unsupervised CL-WSD method exploits the use of monolingual corpora. In this work, we use the \emph{Hamshahri}~\cite{aleahmad2009hamshahri} collection---a widely used monolingual resource for Persian. 

In terms of related work addressing the CL-WSD problem in Persian, Sarrafzadeh et al.~\cite{sarrafzadeh2011} follows a knowledge-based approach by exploiting \emph{FarsNet}~\cite{shamsfard2010semi}---the Persian WordNet. However, since their evaluation collection is not available, the results are impossible to compare with other possible approaches. 


%---a free collection extracted from 1600 movie subtitles. The Parallel English-Persian News (PEN)~\cite{farajian2011pen} corpus aligns 30K sentences of news corpora. However, to the extent of our knowledge, this collections is not yet available. Finally, the collection provided by European Language Resource Association (ELRA) which is a commercial collection with approximately 100K aligned sentences. Among the mentioned resources, TEP is the only publicly available one, but it only contains informal conversations, and therefore it does not provide a general representation of the language.


%In this work, we address this shortage by reporting the result of our unsupervised approach on an standard state-of-the-art benchmark~\cite{rekabsaz2016standard} and compare it with a state-of-the-art CL-WSD system.
